Self Consistent Field Theory of isotropic-nematic interfaces and disclinations in a semiflexible molecule nematic

A Self Consistent Field Theory description of equilibrium, but non uniform, configurations adopted by semi flexible liquid crystal molecules is presented. Two cases are considered, isotropic-nematic phase boundaries, and topological defects in the nematic phase (disclinations). Nematogens are modeled by worm-like chains, with microscopic interaction potential of the Maier-Saupe type, with an added isotropic excluded volume contribution. The thermodynamic fields obtained by numerical minimization of the free energy are the molecular density and the nematic tensor order parameter. Interfaces with both homeotropic and planar alignment are studied, as well as biaxiality and anisotropy around $\pm 1/2$ disclinations. The effects induced by fluid compressibility, interaction strength, and elastic anisotropy that follows from chain flexibility on both types of non-uniform configurations are discussed. Defect core sizes decrease as the system becomes less compressible, eventually reaching a constant value in the incompressible limit. The core size is influenced by the nematic interaction strength and chain persistence length, decreasing as the order increases in the nematic region through manipulation of persistence length and nematic interaction. Additionally, when the far field nematic order is fixed, the core size increases with the persistence length.

==> introduction.tex <==
The anisotropic elasticity of nematic liquid crystals has an important effect on disclination core structure and disclination interactions. This anisotropy arises from the elongated  constituents of the nematic phase, and brings a number of key complications which are not present in the well studied elastically isotropic limit (the so called one constant approximation). Given recent interest in the modeling nematic order in assemblies of the complex microscopic entities that constitute active and biological matter, it is of interest to examine both qualitative and quantitative phenomena that emerge as a consequence of elastic anisotropy.

Within the isotropic elasticity approximation, the topology of defected configurations in two and three dimensional nematic phases is well known, including the case of biaxial ground states \cite{re:alexander12}. In contrast, little is known about director $\hat{\mathbf{n}}$ or tensor order parameter $\mathbf{Q}$ defected configurations that minimize the governing energy under the assumption of anisotropic elasticity. In the special case of isotropic elasticity and in two dimensions, the director angle is a harmonic function of space, and singular defect solutions are well known \cite{re:chaikin95,re:selinger16}. Configurations comprising many defects can be studied via linear superposition, and results have been given for a number of cases of interest, including, for example, binding-unbinding transitions in active matter \cite{re:shankar18}, or defect interactions in complex twisted configurations obtained by conformal mapping techniques \cite{re:tang17}.

Still in two spatial dimensions, but in the case in which splay $K_{1}$ and bend $K_{3}$ elastic constants are different, an analytic -albeit only implicit- solution for the director angle was given by Dzyaloshinskii \cite{re:dzyaloshinskii70,re:hudson89} around an isolated disclination. The director angle differs from the one constant solution in a way that depends only on the azymuthal coordinate around the defect but not on the radial coordinate from the core. Further, the Euler-Lagrange equations derived from the Frank free energy  are not linear, and therefore analytic expressions describing elastic interactions between two disclinations are not known. The case of three spatial dimensions is considerably more complex. In addition to topological charge, a defect line needs to be locally characterized by two vectors: the tangent to the line, and the so called rotation vector $\hat{\Omega}$. In the vicinity of the line core, the rotation vector defines the plane in which the director rotates when encircling the line. Given the added complexity, there are no analytic solutions for the director field around an isolated defect in three dimensions, even in the one constant approximation.

In common thermotropic liquid crystals comprising rod like molecules, the anisotropy contrast between splay, twist, and bend elastic constants is small, and the one constant approximation has been successful in a wide variety of applications. More recently, however, attention has shifted to systems comprised of more complex nematogens and hence the need to explore the properties of anisotropic systems has arisen. For example, in the well studied case of lyotropic chromonic liquid crystals, elastic anisotropy is large. Chromonics encompass a wide variety of soft materials ranging from nucleotides to dyes and pharmaceuticals, and are currently under investigation in a wide range of disciplines \cite{re:lydon10,re:lydon11,re:park08b,re:peng16,re:hiltner21}. A chromonic liquid crystal is a lyotropic mesophase in which the basic
structural unit is a water soluble stack of disk like molecules, with ionic groups on the periphery. The disks assemble in solution into cylindrical aggregates which are bound by weak, non covalent bonds. If the concentration is sufficient, the aggregates align to form either nematic (orientationally ordered fluid) or columnar (semi crystalline) phases. The defining feature that distinguishes chromonics from other lyotropic liquid crystals is the fact that its constituent aggregates can dynamically disassociate under distortion. In these materials, the twist elastic constant is about one order of magnitude smaller than splay or bend \cite{re:zhou12,re:zhou14c,re:zhou17b}.  The splay elastic constant is expected to be linear in the aggregate length, which depends strongly (exponentially) on the scission energy of the stacks comprising the nematogens, itself proportional to the Debye screeening $\lambda_{D}$ (they are weakly charged molecules). The bend constant, which controls aggregate rigidity, scales in these experiments as $\lambda_{D}^{2}$ instead. One manifestation of their unusual structure is the large size of the defect cores in chromomics (tens of microns), as well as their strong anisotropy. A recent study of the fine structure of their disclination cores has revealed the combined presence of anisotropy and biaxiality in the core region of both +1/2 and -1/2 disclinations \cite{re:zhou17}.  Furthermore, and under confinement, they have been shown to exhibit spontaneous chiral symmetry breaking \cite{re:tortora11,re:pellegrino21}. In fact, chromonics are argued to be in a regime in which the classical Ericksen inequalities are violated, yet the twisted ground state is thermodynamically stable for specific choices of the boundary conditions \cite{re:paparini22,re:long23}. Another notable macroscopic manifestation of elastic anisotropy concerns director configurations around disclinations formed in suspensions of flexible biopolymers. Elastic constants of films with a mixture of actin filaments and microtubules assembled in oil-water interfaces have been recently determined  \cite{re:zhang18}. The composition of the mixture was used to tune the ratio of splay to bend elastic constants. Director profiles around disclinations was then fitted to the Dzyaloshinskii solution in order to determine their ratio. The anisotropy contrast studied spans the range of $0.5 < K_{3}/K_{1} < 2.1$ with sufficient differences in the director profile observed to allow a precise measurement of the elastic constant ratio as a function of the mixture composition.

More complex anisotropic effects have been observed in studies of disclination line reconnection in three dimensions \cite{re:zushi22}. It is known that, in two dimensions, anisotropy breaks the symmetry in the motion of +1/2 and -1/2 defects in a configuration of two mutually attracting disclinations. The situation is expected to be qualitatively different in three dimensions as only disclinations of charge 1/2 are expected (unsigned, as opposed to two dimensions), and that can in fact annihilate despite having a charge of the same sign. Nevertheless, the measurement of  disclination separation as a function of time for reconnecting defect lines have revealed that the shortest distance between the two lines still scales as $(t_{0}-t)^{1/2}$ \cite{re:zushi22}, as in two dimensions. For an initially asymmetric configuration containing two wedge disclination segments, symmetry of the director field around the center point between the two disclinations is first established, process that appears to be mediated by a topologically allowed reorientation of the rotation vector $\bm{\Omega}$ of the disclinations. This leads to an energetically favored, symmetric, configuration comprising two twist disclinations instead. It is argued that the fact that all disclination lines observed eventually adopted symmetric twist configurations is a direct consequence of elastic anisotropy (the twist elastic constant is one half of the bend and splay constants in the liquid crystal studied).

While it is possible to study both equilibrium and transient configurations of nematics containing disclinations in the director representation, with the Frank free energy governing elastic distortion, and Leslie-Ericksen hydrodynamics fluid flow, it is often the case that a tensor order parameter representation and the Landau-de Gennes energy are used instead. Virtually all studies of nematic active and biological matter use this representation as it eliminates the need for defect core regularization (specially in three dimensions), and hence it permits a more convenient computational treatment of disclinations and their motion. Unfortunately, this choice has the effect of restricting these studies to the one constant approximation. Elasticity in the tensor order parameter representation is incorporated in a phenomenological series expansion in powers of the order parameter gradient, Eq. \eqref{eq:elastic} below. For small distortions, Frank elastic constants can be related to the coefficients of the expansion as shown in Eq. \eqref{eq:frank-ldg-elastic-comparison}. In order to capture splay-bend anisotropy, the lowest order coefficient that needs to be nonzero, $L_{3}$, is cubic in the order parameter. At this order, the Landau-de Gennes energy is known to become unbounded for any choice of parameters \cite{re:ball10,re:bauman16}. Unboundedness can be traced back to the lack of any constraint in the Landau-de Gennes free energy on the physical admissibility of the eigenvalues of $\mathbf{Q}$. In principle, the requirement of a stable free energy could be accomplished in this case by consideration in the expansion defining ${\cal F}_{el}$ of terms at least of fourth order in $\mathbf{Q}$. However, since there are 22 possible fourth order invariants allowed by symmetry \cite{re:longa87}, the Landau-de Gennes theory becomes intractable for an elastically anisotropic nematic. Building into the theory the constraint that the eigenvalues of $\mathbf{Q}$ must remain within the physically admissible range can be accomplished by an appropriately defined singular potential \cite{re:katriel86,re:ball10,re:schimming20a,re:schimming20b,re:schimming21}. The drawback of this theory is that the determination of the energy needs to be done entirely numerically at an important computational costs relative to simple evaluations of the Landau-de Gennes energy.

Two complementary issues are investigated in relation to elastically anistropic nematic phases, both in the tensor order parameter representation. First, we build on the analysis of Ref. \cite{re:schimming20b} that used a singular potential method to quantitatively describe both bialixiality and anisotropy of disclination cores in chromonics \cite{re:zhou17}. The core is not isotropic, in agreement with earlier predictions  \cite{re:schopohl87}, but rather unixial adopting a so called \lq\lq pancake'' configuration. We use the singular potential method to compute the optical retardance, $\Gamma = S - P$, where $S$ and $P$ are the uniaxial and biaxial order parameters respectively. Exactly at the disclination core, $S = P$, in agreement with experiments and earlier calculations. We then show that as the core is approached $\Gamma_{0} \sim r$, with $\Gamma_{0}$ being the radial component of the Fourier transform of $\Gamma$, and $r$ the radial distance from the core. However, the azymuthal components $\Gamma_{1}$ for a +1/2 disclination and $\Gamma_{3}$ for a -1/2 disclination while nonzero in the biaxial region, they vanish as $r^{2}$ near the core. Hence, while a biaxial region exists separating a far field uniaxial configuration from the uniaxial distribution at the core, which is spatially anisotropic, isotropy is asymptotically restored near the core as the non isotropic components of the azymuthal Fourier transform decay to zero with a higher power of distance.

Second, we focus on the interaction of a pair of disclinations of opposite sign, and examine the nature of their screening at distances much larger than their separation. For isotropic elasticity, the director angle far from the disclination pair behaves as $\theta = q_{1} + q_{2} - d(q_{1}-q_{2}) \sin \varphi/2r$ where $q_{i}$ are the charges of the disclinations separated by $d$, $r$ is the distance from the pair, and $\varphi$ is the azymuth measured relative to the axis defined by the line joining the two defects. For two disclinations of opposite charge, the distortion is screened, and it decays to zero as $1/r$, with an angular dependence given by $\sin \varphi$. The director field for an anisotropic system is more complex, and we compute its angular dependence both near the individual defects and at large distances.  In particular, the far field solution contains an additional term of the form $\pm d \sin (3 \varphi)/r$ that decays with distance with the same power as the isotropic solution, but has a different angular dependence. The sign depends on the particular isomorph of the disclination pair considered. As a consequence, disclination interactions in elastically anisotropic nematics are qualitatively different than their isotropic counterparts, and the implications of these findings on current phenomenology involving multiple defect interactions and motion need to be reexamined.





